Inductive Approach to Cartan's Moving Frame Method with Applications to Classical Invariant Theory

This thesis is devoted to algorithmic aspects of the implementation of Cartan's moving frame method to the problem of the equivalence of submanifolds under a Lie group action. We adopt a general definition of a moving frame as an equivariant map from the space of submanifolds to the group itself and introduce two algorithms, which simplify the construction of such maps. The first algorithm is applicable when the group factors as a product of two subgroups $G=BA$, allowing us to use moving frames and differential invariants for the groups $A$ and $B$ in order to construct a moving frame and differential invariants for $G$. This approach produces the relations among the invariants of $G$ and its subgroups. We use the groups of the projective, the affine and the Euclidean transformations on the plane to illustrate the algorithm. We also introduce a recursive algorithm, allowing, provided the group action satisfies certain conditions, to construct differential invariants order by order, at each step normalizing more and more of the group parameters, at the end obtaining a moving frame for the entire group. The development of this algorithm has been motivated by the applications of the moving frame method to the problems of the equivalence and symmetry of polynomials under linear changes of variables. In the complex or real case these problems can be reduced and, in theory, completely solved as the problem of the equivalence of submanifolds. Its solution however involves algorithms based on the Gr\"obner basis computations, which due to their complexity, are not always feasible. Nevertheless, some interesting new results were obtained, such as a classification of ternary cubics and their groups of symmetries, and the necessary and sufficient conditions for a homogeneous polynomial in three variables to be equivalent to $x^n+y^n+z^n.$

==> abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%% BEGIN ABSTRACT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vskip-2cm


\begin{centering}
{ \large Inductive Approach to Cartan's Moving Frame Method with Applications to
Classical Invariant Theory.}\\
Irina A. Kogan\\
\end{centering}
299  words
\begin{center}   
\Large ABSTRACT
\end{center}

\begin{small}
This thesis is devoted to algorithmic aspects of the implementation of 
 Cartan's moving frame method to the problem of the equivalence of 
submanifolds under a Lie group action. We adopt a general definition of a moving frame 
as an equivariant map from the space of submanifolds to the group itself and 
introduce two algorithms, which simplify the construction of such maps. 
The first algorithm  is applicable when the group  factors as a product of 
two subgroups  $G=BA$,  allowing us to use 
 moving frames and differential invariants  for the groups $A$ and $B$ in order 
to construct
a moving frame and differential invariants for $G$. This approach not only simplifies the
computations, but also produces the relations among the
invariants of $G$ and its subgroups. We use the groups of the projective, the affine and the Euclidean transformations on the plane to illustrate the algorithm. 
We also introduce a recursive algorithm,  allowing, provided  the group action satisfies  certain conditions,
 to construct differential invariants order by order, at each step normalizing more and more of the group parameters, at the end obtaining a moving frame for the entire group. The development of this algorithm has been motivated by the  applications 
of the  moving frame method to the problems of the equivalence and symmetry of 
polynomials under linear changes of variables.  In  the complex or real case these 
problems  can be reduced and, in theory,
 completely solved  as the problem of the equivalence of 
submanifolds.  Its  solution  however involves algorithms based on the 
  Gr\"obner basis computations, which  due to their complexity, are not always feasible. 
Nevertheless, some interesting new  results were obtained, such as a classification  of 
ternary cubics and their groups 
of symmetries, and the  necessary and sufficient conditions for a homogeneous polynomial in three variables to be equivalent to $x^n+y^n+z^n.$   
\end{small}
\vspace*{30pt}
\begin{center}
\rule{6cm}{0.5pt}\\
 Peter Olver\\
\normalsize (Faculty Adviser)
\end{center}
  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% END ABSTRACT%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



